Negative regularity mixing for random volume preserving diffeomorphisms

We consider the negative regularity mixing properties of random volume preserving diffeomorphisms on a compact manifold without boundary. We give general criteria so that the associated random transfer operator mixes $H^{-\delta}$ observables exponentially fast in $H^{-\delta}$ (with a deterministic rate), a property that is false in the deterministic setting. The criteria apply to a wide variety of random diffeomorphisms, such as discrete-time iid random diffeomorphisms, the solution maps of suitable classes of stochastic differential equations, and to the case of advection-diffusion by solutions of the stochastic incompressible Navier-Stokes equations on $\mathbb T^2$. In the latter case, we show that the zero diffusivity passive scalar with a stochastic source possesses a unique stationary measure describing "ideal" scalar turbulence. The proof is based on techniques inspired by the use of pseudodifferential operators and anisotropic Sobolev spaces in the deterministic setting.

==> Outline.tex <==
% !TeX root = prelims.tex


\subsection{Proof of Theorem \ref{thm:AM}}
Here we outline the main steps of Theorem \ref{thm:AM}, leaving the lemmas to be proved in subsequent sections.
The approach is motivated as a combination ideas from \cite{..} and \cite{..}, but with some crucial differences. 

As a first step, we prove that one can obtain annealed mixing in very low regularity starting from $H^{-\delta}$ regularity.
This is proved using the results of \cite{}; see Section \ref{}.
\begin{proposition} \label{prop:LM}
For all $\delta > 0$ sufficiently small, $\exists \gamma_\ell,C_\ell > 0$ such that for all $\kappa\in[0,1]$, and $V(u)$ there holds the following for all $f_0 \in H^{-\delta}$:
\begin{align}
\EE \left[V(u_t)\norm{f_t}_{H^{-100}}^2\right] \leqc_\ell V(u) e^{-\gamma_\ell t} \norm{f_0}_{H^{-\delta}}^2. 
\end{align}
\end{proposition}

The main step is to construct a pseudo-differential operator (PDO) $A_p$ of order $-p$ with symbol $a_p(u) = a_p(u,x,\xi)$ (i.e. depending on the velocity field $u$) such that the following Lasota-Yorke type estimate holds over one time-step, that is, we obtain a contraction up to a more regular error.  
This can be considered somewhat analogous to the quasi-compactness results using a variable order PDO for uniformly hyperbolic maps as in \cite{...}.
However, we work in an annealed setting, that is, the PDO satisfies \eqref{eq:Lasota-Yorke} in expectation -- not pointwise in $\omega$.
This is at the origin of why we can obtain a reasonable result using a PDO which is order $-p$ (not variable order). 
\begin{proposition} \label{prop:LY}
For all $p$ suffiently small, $\exists \gamma_p, C > 0$ such that $\forall \kappa \in [0,1]$,
there exists a symbol $a_p(u,x,\xi)$ (depending on $\kappa$) such tht the pseudo-differential operator $A_p(u) = \mathrm{Op}(a_p(u))$ of order $-p$ and
which satisfies for all initial conditions $u = u_0 \in \mathbf{H}$ and all initial scalar densities $f_0$ the following Lasota-Yorke-type bound
\begin{equation}\label{eq:Lasota-Yorke}
  \E\langle f_1, A_p(u_1)f_1\rangle_{L^2} \leq e^{-\gamma_p}\langle f_0, A_p(u)f_0\rangle_{L^2} + CV(u)\|f_0\|_{H^{-101}}^2. 
\end{equation}
\end{proposition}
Theorem \ref{thm:AM} will follow from Propositions \ref{prop:LM} and \ref{prop:LY} with a suitable
use of the Markov property, the Lyapunov property of $V$ (Lemma \ref{}), and the following Garding's inequality lemma regarding the operator $A_p$.
\begin{lemma} \label{lem:Gard}
There exists constants independent of $\kappa \in [0,1]$ and $u \in \Hbf$ such that for all $f \in H^{-\delta}$ there holds 
\begin{align*}
V(u)^{-1} \norm{f}_{H^{-\delta}}^2 - C V(u) \norm{f}_{H^{-100}}^2 \lesssim \brak{f, A_p(u) f} \lesssim V(u) \norm{f}_{H^{-\delta}}^2. 
\end{align*}
\end{lemma} 
The proof of Lemma \ref{lem:Gard} is carried out in Appendix \ref{} and the proof of Theorem \ref{thm:AM} assuming Propositions \ref{prop:LM} and \ref{prop:LY} and Lemma \ref{lem:Gard} is carried out in Setion \ref{}. 

Now, let us sketch the main idea behind Proposition \ref{prop:LY}. 
The reference \cite{} demonstrated the existence of a $C^1$, strictly positive $\psi_p(u,x,v)$ for $v \in \S^{d-1}$ such that if we denote the tangent (Markov) process by $(u_t,x_t,\xi_t)$ where $\xi_t = (D_x\phi^t_{\omega,u}(x))^T \xi$, then 
\begin{align*}
\tilde{a}_p(u,x,\xi) = \frac{1}{\abs{\xi}^p} \psi_p\left(u,x,\frac{\xi}{\abs{\xi}} \right)
\end{align*}
is an eigenfunction for the tangent Markov semigroup, namely for all $p$ sufficiently small there is a $\Lambda(p) > 0$ such that
\begin{align*}
\EE \tilde{a}_p(u_t,x_t,\xi_t) = e^{-\Lambda(p) t} \tilde{a}_p(u,x,\xi). 
\end{align*}
It is possible to prove \cite{} that $\Lambda(p)$ is the \emph{moment Lyapunov exponent}, namely
\begin{align*}
\Lambda(p) = -\lim_{t \to \infty} \frac{1}{t} \log \EE \abs{D_x \phi^t_{\omega,u} }^{-p}, 
\end{align*}
and that $\Lambda(p) = p \lambda_1 + o(1)$ as $p \to 0$, where $\lambda_1 > 0$ is the top Lagrangian Lyapunov exponent; see e.g. \cite{}.
Moreover, it is possible to prove that (see Lemma \ref{} below) that 
\begin{align*}
V(u)^{-1} & \lesssim \psi_p(u,x,v) \lesssim V(u). 
\end{align*}
Egorov's theorem (Lemma \ref{}) shows that a `wave-packet' of scalar density concentrated in position-frequency phase space at $(x,\xi)$ will be (approximately) mapped to $(\phi^t_{\omega,u}(x), (D_x \phi^t_{\omega,u})^T\xi)$.
For future reference, we denote the tangent bundle mapping $(x,\xi) \mapsto (\phi^t_{\omega,u}(x), (D_x \phi^t_{\omega,u})^T\xi)$ as $T\phi^t_{\omega,u}$. 
Therefore, we can formally expect \eqref{eq:Lasota-Yorke} to hold with $\tilde{a}_p$. 
However, in order to justify this, we first replace $\tilde{a}_p$ with a suitable regularization described in the next lemma. 
\begin{lemma}
For all $\delta > 0$, $\exists a_p^\delta$ such that for each $u$, $a_p^\delta \in \mathcal{S}$ \red{correct PDO symbol class} and which satisfies the following properties: 
\begin{itemize}
\item \red{Estimates correct for the symbol class} 
\item The regularization error estimates 
\begin{align*}
\abs{a_p^\delta(u,x,\xi) - \tilde{a}_p(u,x,\xi)} \leq \frac{\delta V(u)}{\abs{\xi}^p} \\
\frac{1}{2V(u)} a_p^\delta \leq \tilde{a}_p \leq 2V(u) a_p^\delta. 
\end{align*}
\item Lemma \ref{lem:Gard} holds uniformly in $\delta \in (0,1)$.
\item The following version of Egorov's theorem applies: if we define the (random) transfer operator $S^t f := f \circ \phi^t_{\omega,u}$, then there exists a (random) remainder opeartor $R_1$ such that
\begin{align*}
\brak{S^1 f, Op(a_p^\delta) S^1} & = \brak{f, (S^1)^\ast Op(a_p^\delta) S^1 f} \\
& = \brak{f, Op(a_p^\delta(u_1) \circ T\phi^t)f} + \brak{f,R_1^\delta (u) f},
\end{align*}
and that for some $q,b > 0$, 
\begin{align*}
\EE \norm{R_1(u) f}_{L^2}^2 \lesssim \frac{1}{\delta^q} V^b(u) \norm{f}_{H^{-101}}^2. 
\end{align*}
\end{itemize}
\end{lemma}
Finally, we define the symbol $a_p$.
Set $\delta_u := \delta_0 V(u)^{-\alpha}$ for $0 < \delta_0 \ll 1$ and $\alpha > 0$ chosen suitably in the proof and define  
\begin{align*}
a_p(u,x,\xi) := a_p^{\delta_u}(u,x,\xi).
\end{align*}
Note in particular, that the regularization will vary depending on time as $u$ varies. 
It remains to verify Proposition \ref{prop:LY} and Lemma \ref{lem:Gard} for this choice of symbol; this is carried out in Section \red{...}. 
%
%\subsection{Proof of Theorem \ref{thm:UGE}}
%\red{Not sure we really need to include anything about this stuff in the outline...} 
%Here we briefly discuss the proof of Theorem \ref{thm:UGE} and \ref{cor:USM}...e.g. coupling argument + the ``usual'' stability of measures
%
%
%\subsection{Old outline} 
%
%Below I outline the basic steps needed to prove the main result
%\begin{enumerate}
%\item Goal is to construct a pseudo-differential operator $A_p(u_t)$ of order $-p$ (depending on $\kappa$) such that the following Lasota-Yorke type estimate holds at $t=1$
%\begin{equation}%\label{eq:Lasota-Yorke}
%  \E\langle f_1, A_p(u_1)f_1\rangle_{L^2} \leq e^{-\gamma_p}\langle f_0, A_p(u)f_0\rangle_{L^2} + V(u)\|f_0\|_{H^{-101}}^2,
%\end{equation}
%for some $\gamma_p >0$ and $V(u)$ is a suitable Lyapunov function for the $(u_t)$ process, where the constants on the right-hand side don't depend on $\kappa$
%
%\item We build the pseudo differential operator by regularizing an eigenfunction of a certain Feynmann Kac semi-group for the projective process to build a smooth Lyapunov function $a_p$ for the tangent process $(u_t,x_t,\xi_t)$, where $\xi_t = D_x\phi_{u}^t\xi$,
%\[
%  \E a_p(u_t,x_t,\xi_t) \leq e^{-\Lambda(p) t/2} a_p(u,x,\xi).
%\]
%\item We regularize the eigenfunction $\psi_p$ in $x$ by a mollifier $T_\ep \psi_p$ such that
%\[
%  \|\psi_p - T_\ep \psi_p\|_{C_V} <\ep \|D \psi_p\|_{C_V} \leqc \ep
%\]
%Note the estimate is uniform in $\kappa$ since $\psi_p\in$ is uniformly bounded in $C^1_V$.
%For each $\ep>0$ we can get the bound (using twist bounds)
%\[
%  \E|\xi_t|^{-p}(T_{\ep}\psi_p(u_t,x_t,\xi_t/|\xi_t|)) \leq e^{-\Lambda(p) t}|\xi|^{-p}T_{\ep}\psi_p(u,x,\xi/|\xi|) + \ep C V(u)|\xi|^{-p}T_{\ep}\psi_p(u,x,\xi/|\xi|)
%\]
%and therefore choosing $\ep(u) \sim V(u)^{-1}$ small enough and defining $a_p(u,x,\xi) = |\xi|^{-p}T_{\ep(u)}\psi_p(u,x,\xi/|\xi|)$ gives the Lyapunov estimate. Note that with this choice of regularization, we have that
%\[
%  |D_{x,\xi}^ka_p| \leqc |\xi|^{-p -k} V(u)^{k+1}.
%\]
%
%
%\item (G\r{a}rding's inequality step) Using upper and lower bounds on $\psi_{p}$ the PDO $A_p = a_p(u,x,D)$ will satisfy the following quantitative version of G\r{a}rding's inequality for $p\in (0,1)$
%\[
%  V(u)^{-1}\|f\|_{H^{-p/2}}^2 - C V(u)^{101}\|f\|_{H^{-101}}^2 \leqc \langle f, A_p(u)f\rangle \leqc V(u) \|f\|_{H^{-p/2}}^2
%\]
%where the constants are independent of $\kappa$.
%
%{\color{red} May need the Lyapunov functions here to have different parameters?}
%
%\item (Egorov's Theorem Step) Next we consider $S^{t} f = f\circ (\phi^{t,\kappa}_\omega)^{-1}$ the transfer operator associated to the SDE suitably extended to $H^{-\delta}$ ($\kappa$ and $\omega$ dependence are suppressed for brevity), then we show that for $t=1$ we have
%\[
%\left((S^{1})^{*}A_p(u_t) S^{1}\right) = \mathrm{Op}(a_p(u_1)\circ T\phi^{1,\kappa}_{u,\omega}) + R_1(u),
%\]
%
%where $R_1(u)$ is a random PDO order $-p-1$ and satisfies the following uniform in $\kappa$ estimate
%\[
%  \E|\langle R_1(u)f,f\rangle| \leqc V(u)\|f\|_{H^{-(p+1)/2}}.
%\]
%By interpolation and G\r{a}rding's inequality we have for $\ep>0$
%\[
%  \E|\langle R_1(u)f,f\rangle| \leq \ep \langle f, A_p(u) f\rangle + C_\ep V(u)^{200}\|f\|_{H^{-101}}^2. 
%\]
%
%\item The Lasota Yorke estimate now follows from Egorovs theorem and the Lyapunov estimate choosing $\ep$ small enough
%\begin{equation}
%\begin{aligned}
%  \E\langle S^{1} f,  A_p(u_1)S^{1} f\rangle_{L^2} &= \E\left\langle f, \left((S^{1})^{*}A_p(u_1)S^{1}\right)f\right\rangle_{L^2}\\
%   &= \left\langle f, \mathrm{Op} (\E a_p(u_1,x_1,\xi_1))f\right\rangle_{L^2} + \E \langle f, R_1(u) f\rangle_{L^2}\\
%   &\leq e^{-\Lambda(p)/3}\langle f, A_p(u) f\rangle + C V(u)^{200}\|f\|_{H^{-101}}^2
%   \end{aligned}
%\end{equation}
%
%\item We now want to iterate this bound. To do this, we let $G(u,f) = \langle f, A_p(u)f\rangle$ and $H(u,f) = V(u)\|f\|_{H^{-101}}^2$ so that the Lasota Yorke inequality reads
%\[
%  P_1G \leq e^{-\Lambda(p)/3}G + C H,
%\]
%where $P_t$ is the Markov semi-group for the $(u_t,S^tf)$ process. Iterating this yields
%\[
%  P_n G \leq e^{-n\Lambda(p)/3}G + \sum_{k=1}^n C e^{-(n-k)\Lambda(p)/3} P_kH.
%\]
%
%\item Next we need to show that $P_k H$ decays exponetially fast if we give up some regularity. Namely we show that two point geometric ergodicity implies the following estimate
%\[
%  \E V(u_t)\|S^tf\|_{H^{-101}}^2 \leq V(u) e^{-t \mu}\|f_0\|_{H^{-p/2}}^2
%\]
%for some $\mu$ (independent of $\kappa$) if $p$ is chosen small enough $0\leq p \ll 1$.
%
%\item Substiting this into the iterated estimate yields our 
%\[
%  \E \langle S^nf, A_p(u_n) S^nf\rangle \leq e^{-\Lambda(p) n/3 } \langle f, A_p(u)f\rangle + C V(u) e^{- n \mu}\|f\|_{H^{p/2}}^2
%\]
%\item Finally using G\r{a}rding and the decay estimate again yields
%\[
%\begin{aligned}
%  \E V(u_n)\|S^nf\|_{H^{-p/2}}^2 &\leq e^{-n\Lambda(p)/3}\|f\|_{H^{-p/2}}^2 + \E V(u_n)\|f_n\|_{H^{-101}}^2 + C V(u)e^{-n \mu}\|f\|_{H^{-p/2}}\\
%  &\leq e^{-n\Lambda(p)/3}\|f\|_{H^{-p/2}}^2 + C V(u) e^{-n\mu}\| f\|_{H^{-p/2}}\\
%  &\leqc V(u) e^{-n \mu^\prime} \|f\|_{H^{-p/2}}^2,
%\end{aligned}
%\]
%where $\mu^\prime = \min\{\Lambda(p)/p, \mu\}$.
%
%\item Finally we need to go from discrete to continuous time. Which just requires a time 1 bound in expectation for $S^t$.
%
%
%\end{enumerate}
%
%\subsection{A time-infinitesimal approach to getting higher moments and Egorov}
%Below we sketch an approach to getting higher moments using time infinitesimal estimates and the generator. This proof essentially combines the proof of Egorov's theorem, and the iteration step in one estimate
%
%Let $f_t = S^t f_0 = f_0\circ \phi^t$ and denote
%\[
%  G(u,f) = \langle f, A_p(u) f\rangle.
%\]
%Then we have for $G_t = G(u_t,f_t)$
%\[
%  \partial_t G_t = \langle f_t, [u_t\cdot \nabla,A_p(u_t)] f_t\rangle + \langle f_t, \mathrm{Op}(\mathcal{L}_u a_p)f_t\rangle + \partial_t M_t
%\]
%where $M_t$ is a martingale whose quadratic variation is controlled by
%\[
%  \sum_k\int_0^t\langle f_s, \mathrm{Op}(D_{u_k}a_p(u_s))f_s\rangle^2\ds \leqc \int_0^t V(u_s)^2\|f_s\|_{H^{-p/2}}^4\ds
%\]
%and $\mathcal{L}_u$ is the generator of the fluid motion. The idea behind the proof of Egorov's theorem is that
%\[
%  \sigma\left([u\cdot \nabla,A_p(u)]\right) \sim \sum_{\alpha \geq 0} \frac{i^{\alpha}}{\alpha!} \left[D^\alpha_\xi(u\cdot i\xi) D_x^\alpha a_p - D^\alpha_x(u\cdot i\xi)D^{\alpha}_\xi a_p\right] = -\{H_u,a_p\} + R_u
%\]
%where $R_u\in S^{-p-1}_{1,0}$ uniformly in $\kappa$ and satisfies $|\sigma(R_1)|\leq |\xi|^{-p-1}V(u)^2$, and $H_u(x,\xi) = (u(x)\cdot \xi)$ is a Hamiltonian assocaited with the velocity $u$ lifted to tangent bundle.
%
%Now we know from the fact that 
%\[
%  \E a_p(u_t,x_t,\xi_t) \leq e^{-\Lambda(p)t/3} a_p(u,x,\xi)
%\]
%and the positivity of $a_p$ that
%\[
%  \{H_u,a_p\} + \mathcal{L}_u a_p \leq - (\Lambda(p)/3)a_p.
%\]
%Using this with the bound on $R_u$, and interpolating to $H^{-101}$ gives
%\[
%  \partial_t G_t \leq - (\Lambda(p)/4) G_t + V(u_t)^{202}\|f_t\|_{H^{-101}}^2 + \partial_t M_t. 
%\]
%Naturally to get higher moments in $G$, we need to apply It\^o's formula for $m \geq 1$
%\[
%\partial_t G^m_t \leq -(m\Lambda(p)/4) G_t^m + m V(u_t)^{202}\|f_t\|_{H^{-101}}^{2}G^{m-1}_t + C_m G^{m-2}_tV(u_t)^2\|f_t\|_{H^{-p/2}}^4 + \partial_t M_G(t).
%\]
%
%{\color{red} The stuff below is wrong}
%Integrating this and using the Martingale property gives
%\[
%  \E G^m_t \leq e^{-\gamma t} G_0^m + C \int_0^t e^{-\gamma(t-s)} \E V(u_s)^{202m}\|f_s\|_{H^{-101}}^{2m}\ds, 
%\]
%where $\gamma = m \Lambda(p)/5$.
%
%The proof will be complete if we can show that
%\[
%  \E V(u_t)^{202m}\|f_t\|_{H^{-101}}^{2m} \leq C e^{-\mu t} V(u)^{202m}\|f_0\|_{H^{-p/2}}^{2m}.
%\]
%
%


% \subsection{Regularization procedure}
% We now explain how to use the Lasota Yorke estimate \eqref{eq:Lasota-Yorke} to prove the annealed estimate. 

% To see this, we let $T_\ep$ be a mollifier and note that
% \begin{equation}
% \begin{aligned}
%   \E\|M_pS^{t,\kappa}(I- T_\ep) f_0\|^2_{L^2} &\leq e^{-\Lambda(p)t}\|M_p(I-T_\ep) f_0\|_{L^2}^2 + C(u)\|(I-T_\ep) f_0\|_{H^{-(p+1)/2}}^2\\
%   &\leq e^{-\Lambda(p)t}\|f_0\|_{H^{-p/2}}^2 + C(u)\ep\|f_0\|_{H^{-p/2}}^2
% \end{aligned}
% \end{equation}
% Therefore using our uniform in $\kappa$ mixing result
% \begin{equation}
% \begin{aligned}
% \E\|M_pS^{t,\kappa}f_0\|_{L^2}^2 &\leqc \E\|M_pS^{t,\kappa}(I-T_\ep)f_0\|_{L^2}^2 + \E\|M_pS^{t,\kappa}T_\ep f_0\|_{L^2}^2\\
% &\leqc e^{-\Lambda(p)t}\|f_0\|_{H^{-p/2}}^2 + C(u)\ep\|f_0\|_{H^{-p/2}}^2 + V(u)e^{-\gamma t}\|T_\ep f_0\|_{H^{p/2}}^2\\
% &\leqc e^{-\Lambda(p)t}\|f_0\|_{H^{-p/2}}^2 + C(u)\ep\|f_0\|_{H^{-p/2}}^2 + V(u)e^{-\gamma t}\ep^{-p}\|f_0\|_{H^{-p/2}}^2
% \end{aligned}
% \end{equation}
% Choosing $\ep= e^{-\alpha t}$, we obtain
% \[
%   \E\|M_pS^{t,\kappa}f_0\|_{L^2}^2 \leqc V(u)e^{-\beta t}\|f_0\|_{H^{-p/2}}^2.
% \]
% where $\beta = \min\{\Lambda(p),\alpha,\gamma-p\alpha\}$ choosing $\alpha < \gamma/p$ ensures that $\beta >0$ 


==> PDOs_on_torus.tex <==
%!TEX root = main.tex

% Following Pflaum, or Faure-Roy-Sjostrand, we can quantize symbols  $a : T^*M \to \mathbf C$ (can also take $a$ to be defined on a vector bundle) by taking a cutoff $\chi : TM \to [0,1]$ which is identically 1 near the zero section $0_{TM}$, and use the normal map to define coordinates and local fourier transforms.. On the torus, this procedure can be simplified quite a bit, and we can define $Op(a)$ as follows. Let $\chi : \mathbf R^d \times \mathbf R^d \to [0,1]$ be a cutoff for which $\chi(x,y) =  1$ for all $|x-y| < \delta$ for some $\delta$, and 0 for all $|x-y| > \delta'$ for some $\delta'> \delta$.  We also require that $\chi(x + k, y+ k) = \chi(x,y)$ for all $k \in \mathbf Z^d$.  More conveniently, one can take $\chi(x,y) = \chi_1(x-y)$. Then, we can define
% \[
% Op_\chi(a)f(x) := \int_{\mathbf  R^d \times \mathbf R^d} e^{i(x-y)\xi} a(x,\xi)  \chi(x,y)f(y)d\xi dy.
% \]
% Observe that the kernel $K_\chi (x,y) := \int_{\mathbf  R^d} e^{i(x-y)\xi} \chi(x,y) a(x,\xi) d\xi$ is smooth outside the diagonal $x = y$. Thus, for any two cutoffs $\chi,\tilde \chi$,  the operator $Op_\chi (a) - Op_{\tilde \chi}(a)$ is infinitely smoothing, i.e. it maps $\mathcal E' \to \mathcal E$. This is how we can get quantization ``up to smoothing" operators. This will be useful in Egorov's theorem, when we must evaluate the difference of quantization between the cutoffs $\chi(\Phi(x),\Phi(y))$ and $\chi(x,y)$.



==> regularization.tex <==
%!TEX root = main.tex

Let $S^{t}$ be the semigroup induced by a random vector field $u$. Originally, the idea was to construct the psuedo-differential operator $Op(a_p)$, with the symbol $a_p = |\xi|^{-p} \psi_p(u,x,\xi)$. However, there are issues associated with the limited regularity of $\psi_p$.

To get around this, we work with a mollified version of the symbol. Once again I will ignore the dependence on $u$ for convenience.
Let $\psi_p^\delta$ be a $C^\infty$ approximation of $\psi_p$ in $x$ and $\xi$, satisfying
\[
\|\psi_p ^\delta - \psi_p\|_{L^\infty(\mathbb T^d\times \mathbb S^{d-1})} \leq \delta.
\]
Let $a_p ^\delta =|\xi|^{-p}\psi_p$. Observe that for all $(x,\xi) \in T^*\mathbb T^d  =\mathbb T^d \times \mathbb R^d$,
\[
|a_p^\delta(x,\xi) - a_p(x,\xi)| \leq \frac{\delta}{|\xi|^p}.
\]
Then, let $\tilde \phi^t$ be the flow map lifted to $T^*\mathbb T^d$.  The symbol $a_p$ then enjoys the pointwise bounds
\begin{align}
\mathbb  E[a_p^\delta \circ \tilde \phi^t(x,\xi)]& \leq \mathbb  E[a_p \circ \tilde \phi^t(x,\xi)] + \mathbb  E[(a_p -a_p^\delta)\circ \tilde \phi^t(x,\xi)] \\
&\leq e^{-\Lambda(p)t} a_p(x,\xi) +\mathbb  E\left[\frac{\delta}{|(D\phi^t(x))^{-T} \xi|^p}\right]\\
&\leq e^{-\Lambda(p)t} a_p^\delta(x,\xi)  + \delta \left ( \frac{e^{-\Lambda(p)t} }{|\xi|^p} +\mathbb  E\left[\frac{1}{|(D\phi^t(x))^{-T} \xi|^p}\right]\right)
\end{align}
Let $K_1 ,K_2\geq1$ be constants such that for all $(x,v) \in \mathbb T^d \times \mathbb S^{d-1}$,
\begin{align}
\frac{1}{K_1} \leq \psi_p(x,v) \leq K_1, \quad \frac{1}{K_2} \leq \mathbb  E[(D\phi^1(x))^{-T}v] \leq K_2
\end{align}
Taking $\delta $ small enough depending on $K_1$, we guarantee
\[
\frac{1}{2} a_p^\delta \leq a_p \leq 2 a_p^\delta , \quad 
\]
Then, continuing the bounds on $\mathbb E[a_p^\delta \circ \tilde \phi^t(x,\xi)]$ from earlier in the case $t= 1$, we have
\begin{align*}
\mathbb E[a_p^\delta \circ \tilde \phi^1(x,\xi)]&\leq e^{-\Lambda(p)} a_p^\delta(x,\xi) + \delta (1+ K_2^p) \frac{1}{|\xi|^p} \\
&\leq e^{-\Lambda(p)} a_p^\delta(x,\xi)  +  2\delta K_2^pK_1 a_p(x,\xi)\\
&\leq (e^{-\Lambda(p)}  +  4 \delta K_2^p K_1) a_p^\delta(x,\xi).
\end{align*}
One can prove an analogous lower bound, with the term $4\delta K_2^p K_1$ subtracted instead, i.e.
\begin{align*}
e^{-\Lambda(p)-O(\delta)}a_p^\delta(x,\xi) \leq \mathbb E[a_p^\delta \circ \tilde \phi^1(x,\xi)]\leq e^{-\Lambda(p)+O(\delta)}a_p^\delta(x,\xi).
\end{align*}
With the symbol $a_p^\delta$, we can more easily construct psuedo-differential operators with good remainder terms, etc. than we would be able to with $a_p$. This comes at the cost of perturbing the rate of decay, but this seems necessary anyway.

Regarding $u$ dependence, this enters into the argument in two ways: 1) mollification of $\psi_p$ and the size of $K_1$, both of which depend on the  size of the $C^1$ norm of $\psi_p$; 2) the size of $K_2$. Hopefully you (Sam or Jacob) can help here!


